NetRCA: An Effective Network Fault Cause Localization Algorithm

Localizing the root cause of network faults is crucial to network operation and maintenance. However, due to the complicated network architectures and wireless environments, as well as limited labeled data, accurately localizing the true root cause is challenging. In this paper, we propose a novel algorithm named NetRCA to deal with this problem. Firstly, we extract effective derived features from the original raw data by considering temporal, directional, attribution, and interaction characteristics. Secondly, we adopt multivariate time series similarity and label propagation to generate new training data from both labeled and unlabeled data to overcome the lack of labeled samples. Thirdly, we design an ensemble model which combines XGBoost, rule set learning, attribution model, and graph algorithm, to fully utilize all data information and enhance performance. Finally, experiments and analysis are conducted on the real-world dataset from ICASSP 2022 AIOps Challenge to demonstrate the superiority and effectiveness of our approach.

==> 2_related_work.tex <==
\section{Related Work}\label{sec:related}
%(Qingsong, Liang)

% existing work include adaptive root cause analysis~\cite{mfula2017adaptive}, on unsupervised techniques~\cite{gomez2015automatic}, using temporal analysis ~\cite{munoz2016root}.

In this section, we briefly review some related work in automatic root cause analysis, with an emphasis on temporal methods, unsupervised methods, Bayesian networks, and explainable methods. 

As a major data source is the key performance indicator (KPI) monitoring data in the time series format, a key challenge is how to utilize these time-series metric data effectively. In \cite{munoz2016root}, it proposes an automatic diagnosis algorithm to analyze the temporal evolution of a plurality of metrics and searches for potential interdependence under the presence of faults. Basically, it computes the similarity in time between metrics and then compares it with stored patterns to determine the root cause of the fault. As it relies on a set of stored patterns, the label information is crucial for success. Recently, CloudRCA~\cite{zhang2021cloudrca} is proposed for root cause analysis via robust time series analysis, including robust periodicity detection~\cite{wen2021robustperiod}, robust and efficient seasonal-trend decomposition~\cite{wen2019robuststl,yang2021robust}. 

The unsupervised method is a good choice, especially when the labeled data is limited. In \cite{gomez2015automatic}, it proposes an automatic diagnosis system based on an unsupervised algorithm self-organizing maps (SOMs). It intends to refine the diagnosis solution provided by the traditional SOM according to the so-called
silhouette index and the most similar cause based on the
minimum Xth percentile of all distances. 

In the literature, the Bayesian networks~\cite{cai2017bayesian} are proposed to perform reasoning for automatic diagnosis. Unfortunately, due to the diverse data source and size, the resulting network must consider all possible states of each node and their associated probabilities, making network learning challenging. In \cite{mfula2017adaptive}, it proposes an automated fault detection and diagnosis solution called adaptive root cause analysis (ARCA), which uses measurements and other network data together with Bayesian network theory to perform automated evidence-based RCA.

Recently, the explainability of artificial intelligence (AI) is more concerned as it can provide insights into the decision made by AI so humans can understand. In ~\cite{terra2020explainability}, proposes the application of multiple global and local explainability methods with the main purpose of root cause analysis in a 5G network by identifying important features contributing to the decision. The applied XAI methods include SHAP, permutation importance (PI), LIME, and causal dataframe to validate the causality of the important features. Although it is an interesting application, the application of XAI methods in root cause analysis is shallow. 




% more can be found in the review work~\cite{mulvey2019cell}

%in Microservice Environments: 
%MicroRank~\cite{yu2021microrank}, 
%MicroRCA~\cite{wu2020microrca},
%MicroCause~\cite{meng2020localizing},





 % ServiceRank~\cite{ma2021servicerank},




==> bak_intro.tex <==
\section{Introduction}
(by Liang)

aim:
detecting changes of variance (CoV) assuming that the variance function can be described by a piecewise constant function with segments delimited by unknown change-points.
In practice, we aim to the CoV is resilient to departures from the assumption of normality or presence of outliers.

Whilst considerable research effort has been given to the change in mean problem, the detection of changes in variance has received comparatively fewer attentions~\cite{JSSv058i03}.


change point detection received lots of research interests in signal processing  \cite{Ding2017} \cite{VincentBookQuickDetect2008}, \cite{Lung-Yut-Fong2011}, and data mining society \cite{Aminikhanghahi2017}

Change of variance is important in time series analysis.
\cite{Tsay1988}

With application in different disciplines, like in signal processing \cite{Wahlberg2011}, \cite{Lau2017}, \cite{Galleani2014}, applied statistics \cite{EJASA16793}, Economic statistics \cite{Xu2016}, oceanography \cite{Killick2010}, 

Method
Use of cumulative sum to detect Change of variance 
\cite{Inclan1994}


STL method
STL~\cite{STL_cleveland1990stl}, RobustSTL~\cite{RobustSTL_wen2018robuststl}, and TBATS~\cite{TBATS_de2011forecasting}.

Trend filtering
H-P filter \cite{hp_hodrick1997}, L1 trend filter \cite{L1trend_kim2009ell}, RobustTrend filter \cite{WenRobustTrend19}



In the formulation, the variance filtering is close related to covariance fitting \cite{stoica2005spectral}



we adopt robust statistics \cite{huber2009robust}
